Neutaint: Efficient Dynamic Taint Analysis with Neural Networks

Dynamic taint analysis (DTA) is widely used by various applications to track information flow during runtime execution. Existing DTA techniques use rule-based taint-propagation, which is neither accurate (i.e., high false positive) nor efficient (i.e., large runtime overhead). It is hard to specify taint rules for each operation while covering all corner cases correctly. Moreover, the overtaint and undertaint errors can accumulate during the propagation of taint information across multiple operations. Finally, rule-based propagation requires each operation to be inspected before applying the appropriate rules resulting in prohibitive performance overhead on large real-world applications. In this work, we propose NEUTAINT, a novel end-to-end approach to track information flow using neural program embeddings. The neural program embeddings model the target's programs computations taking place between taint sources and sinks, which automatically learns the information flow by observing a diverse set of execution traces. To perform lightweight and precise information flow analysis, we utilize saliency maps to reason about most influential sources for different sinks. NEUTAINT constructs two saliency maps, a popular machine learning approach to influence analysis, to summarize both coarse-grained and fine-grained information flow in the neural program embeddings. We compare NEUTAINT with 3 state-of-the-art dynamic taint analysis tools. The evaluation results show that NEUTAINT can achieve 68% accuracy, on average, which is 10% improvement while reducing 40 times runtime overhead over the second-best taint tool Libdft on 6 real world programs. NEUTAINT also achieves 61% more edge coverage when used for taint-guided fuzzing indicating the effectiveness of the identified influential bytes.

==> motivation.tex <==
\section{Motivation}
\label{sec:Motivation}
In this section, we show three fundamental problems in the design and implementation of taint: under-taint, over-taint, and large runtime overhead. Even with the heavy instrumentation that causes these large runtime overheads, manually engineered rules for taint propagation still have poor accuracies in capturing information flows, implying an alternative lightweight mechanism to track information flows is desirable. These limitations of taint severely limit its applicability to real-world programs.

\subsection{Under Taint Issue}

\subsection{Over-Taint Propagation}

\subsection{Overhead}



==> overview.tex <==
\subsection{Overview}

1) The way to do neural taint. 2) Accuracy and interpretability of Neural taint. Neural taint is more accurate, and thus more interpretable than traditional taint. 3) Application of Neural taint, fuzzing. Fuzzing is one of the most widely-used and important applications of taint.(put into background)

The aim of Dynamic taint analysis is to find hot bytes that affect program behaviors. Our method infers these hot bytes from a neural network model rather than dynamically propagating taint flow at runtime. 
First, for a given program and a set of inputs, 
we track and mark the program branches that are executed 
while running the program using those inputs. 
These branches represent the dynamic behavior of the program. 
Next, we build a neural network model (NN) to learn the 
dynamic behavior\textemdash given a program input, the 
NN learns and then can predict which branches will be executed. The NN model makes the predictions based on different values of input features. The more important a feature is, the more greatly it would affect the NN output. For our neural network model, the more important feature which affect the program behaviors are those hot bytes. We identify these hot bytes by constructing an adversarial saliency map which indicate the most important features.

%However, predicting a diverse set of branches accurately from 
%%%(\eg 
%%%%In particular, if a branch is far from the branches that the model has already seen during training, it is very difficult to predict the distant branches accurately. To address this problem, we use an incremental learning setting: we use an already trained NN to guess which input values are more likely to change the branching behavior of the program by following the NN's gradients. These locations are called  {\em hot bytes}. \yizheng{To explain NN's decision using gradient, is this sensitivity? Saliency Method? Different from what people call ``attribution''?} 
%Next, we further mutate those locations to generate new inputs and gather new branching behavior by running the program with those inputs. We further train the model with these new inputs and the corresponding branches. In particular, we only train on the inputs that have covered at-least one new branch to reduce over fitting. 
%With such incremental learning setting, the NN can approximate a diverse dynamic behavior of the program.

%The rest of the section illustrates each of these steps in details.

%Then we identify hot bytes by computing the top-k gradient of final layer output with respect to neural network input. 
%The hot bytes are approximated taint locations of program inputs. 
%For further analysis, we could generate a richer sampling dataset by mutating inputs on hot bytes. After checking interesting program behaviors of these mutated inputs on target program, we could filter out representative inputs which explore unique program behaviors and perform incremental learning to refine our neural program. 

\begin{figure}[h]
\centering
%\framebox[4.0in]{$\;$}
%\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[scale=0.5]{./fig/overview.pdf}
\caption{\textbf{\small CHANGE ME>>>An overview of our approach.}}
\label{fig:overview}
\end{figure}

